DYNOTEARS: Structure Learning from Time-Series Data

We revisit the structure learning problem for dynamic Bayesian networks and propose a method that simultaneously estimates contemporaneous (intra-slice) and time-lagged (inter-slice) relationships between variables in a time-series. Our approach is score-based, and revolves around minimizing a penalized loss subject to an acyclicity constraint. To solve this problem, we leverage a recent algebraic result characterizing the acyclicity constraint as a smooth equality constraint. The resulting algorithm, which we call DYNOTEARS, outperforms other methods on simulated data, especially in high-dimensions as the number of variables increases. We also apply this algorithm on real datasets from two different domains, finance and molecular biology, and analyze the resulting output. Compared to state-of-the-art methods for learning dynamic Bayesian networks, our method is both scalable and accurate on real data. The simple formulation and competitive performance of our method make it suitable for a variety of problems where one seeks to learn connections between variables across time.

==> aupr_table_small.tex <==

\begin{tabular}{l|c}

\toprule

  Algorithm &  Average \\
 {} &  AUPR \\


\midrule
    \textbf{DYNOTEARS} &         \textbf{0.173} \\
		G1DBN &         0.110 \\
		ScanBMA &       0.101 \\
		VBSSMb &        0.096 \\
		VBSSMa &        0.086 \\
    Ebdbnet &       0.043 \\
\bottomrule

\end{tabular}

